Verifying Reachability in Networks with Mutable Datapaths

Recent work has made great progress in verifying the forwarding correctness of networks . However, these approaches cannot be used to verify networks containing middleboxes, such as caches and firewalls, whose forwarding behavior depends on previously observed traffic. We explore how to verify reachability properties for networks that include such "mutable datapath" elements. We want our verification results to hold not just for the given network, but also in the presence of failures. The main challenge lies in scaling the approach to handle large and complicated networks, We address by developing and leveraging the concept of slices, which allow network-wide verification to only require analyzing small portions of the network. We show that with slices the time required to verify an invariant on many production networks is independent of the size of the network itself.

==> hloutline.tex <==
\section{Extremely High Level Outline}
\begin{outline}
\1 Middleboxes prevalent, more common with NFV - need to be able to verify that a combination of middleboxes in a network implement desired high-level policies.
\1 Verification is hard in the presence of stateful middleboxes: must consider how state evolves.
%    \2 Focus here on isolation invariants: data and node level isolation.
\1 Here we present some techniques for verifying networks with middleboxes, three main ideas for scalability:
    \2 Use limited high-level models of middleboxes which specify behavior: makes verification tractable in the presence of several middleboxes in a network.
    \2 Define some principles for how to design and combine middleboxes in a way that simplifies verification (RONO).
    \2 Verify implementation by observing middlebox behavior and enforcing that this behavior is a subset of specification behavior.
\1 How to specify middleboxes
    \2 Specified using a limited grammar that is equivalent to state machine with timed transitions.
        \3 For simplicity we express them as programs that are able to
            \4 Receive packets
            \4 Send packets
            \4 Write data into dictionaries.
            \4 Read from dictionaries
            \4 Construct new packets.
            \4 Use conditionals (if-statements).
        \3 This has some important limitations
            \4 No input dependent loops: we only assume fixed processing steps for a packet.
            \4 Hard to express some other kinds of processing.
        \3 Assert that for most middleboxes this is fine.
            \4 Even for complex processing for classification as is done by DPI can divide middlebox into a part that runs complex classification
            and part that then uses this classification to actually update middlebox state and send out packets.
            \4 Express complex classification algorithm as an uninterpreted function with a given range of outputs.
            \4 During verification check if any of the range of outputs can result in a violation.
    \2 Can convert this specification into two things
        \3 A set of formulas that can be checked using an SMT solver
        \3 Functional code for verifying runtime behavior.
    \2 Unfortunately limited grammar alone is not sufficient.
        \3 Cannot provably show that isolation is decidable on all combinations of such middleboxes.
        \3 Need an additional assumption: require middleboxes to be ``local''.
           \4 Locality here implies that a middleboxes decisions depend only on either data contained within the packet being processed or local state
            based on previously received packets. \fixme{Constants are fine too}.
            \4 Given this assumption can convert occurrences of $\exists$ to a function, our formulas are equivalent to the Effectively Propositional (EPR)~\cite{} fragment of
            first-order logic which is guaranteed to be computable.
\1 Our verification problem is now:
    \2 A set of middlebox definitions as above.
    \2 Network that can be analyzed using VeriFlow.
    \2 Use VeriFlow to compute service chains, describing order in which packets traverse middleboxes.
    \2 Combine middlebox formulas with this traversal to get a formula for the network/paths that need to be analyzed.
    \2 Verify properties here.
\1 Given simple middlebox models we have:
    \2 Verifying networks with full middlebox is very expensive
    \2 Verifying networks with simplified middlebox model is simpler, faster. Complexity \fixme{something}.
    \2 Next we talk about a property RONO. With RONO verifying a given path is sufficient to prove an invariant. Cheaper than proving for whole network.
        \3 RONO for a middlebox implies correct behavior of middlebox depends only on flow state.
        \3 Can consider a middlebox to be several parallel instances that can be examined in isolation.
        \3 Some composition of middleboxes is also RONO: parallel composition always RONO, sequential composition RONO if meets requirements.
    \2 There are a set of invariants that are RONO-complete, \ie can always be implemented in a RONO manner.
        \3 For instance, static isolation invariants: need to add firewall, don't rely on global information.
        \3 Here we focus on static isolation invariants.
        \3 Always provide a mechanism that can be enforced statically.
\eat{
\1 Verification as above is still hard. Turns out many middleboxes and combinations can be analyzed in isolation
    \2 Call this property RONO. Implies, a single middlebox (or a combination) can be considered as several parallel middleboxes.
    \2 Correctness depends only on per-flow state or flows between two specific end hosts etc.
    \2 Talk about combination and what not being RONO implies.
}
\1 Finally, to check implementation we can use functional code to verify runtime behavior.
    \2 Code is very simple: only includes middlebox behavior.
    \2 RONO again helps simplify verification: can parallelize verification code easily.
\1 Discussion + summary
\end{outline}

==> notes.tex <==
\section{Notes}
These are note from the many rejections, enumerating some points we should make sure we include in the text. I think many of these are already in the text, but just noting these here so we can be sure.

\subsection{Problem}
\begin{outline}
\1 Large numbers of middleboxes deployed in operational networks, often for security and performance.
    \2 Usually everyone deploys a few common kinds of middleboxes: firewalls, caches, IDSes, etc.
\1 Middleboxes result in some new kinds of behaviors, which can affect network verification in four ways:
    \2 The classification algorithm can be very complicated; in particular can look at payloads (IDS), compute hashes (load balancers), rely on complex match algorithms (regex matches in IDS).
    \2 Can overwrite packet fields (NATs) which might affect the behavior of downstream middleboxes.
    \2 Do more than just forward packets, \eg caches are terminating middleboxes, receiving a request might result in the cache establishing a new flow to the origin.
    \2 Are stateful which means: state established by a packet earlier in the flow can affect all later packets (learning firewall), and state established by one flow affects the behavior of another (IDS, caches). 
\1 The first two of these problems are actually not restricted to middleboxes.
    \2 Addressed by HSA, VeriFlow, etc. too. They increase verification complexity (since is function of number of bits/fields examined).
\1 The last two require network administrators and verification tools to reason across packets and flows.
    \2 Whether a connection is allowed or not depends on previous packets (firewall) or connections (IDS). 
        \3 This means the behavior of the network itself depends on a potentially unbounded sequence of packets received so far.
        \3 Furthermore, network administrators must therefore be able to check invariants which depend on past behavior (e.g., can A send data to B without B establishing a connection, can A send data to B when A is known to cause a DoS attack, etc.).
    \2 The lifetime of data in the network is decoupled from the lifetime of the connection, \eg data might be cached at a cache.
        \3 Behavior of one flow might be affected by another, existing dataplane verification tools do not perform such cross-flow analysis. \fixme{Example where this really matters and is not just a binary choice.}
        \3 It is useful to therefore reason about who can access data \fixme{cite \url{https://goo.gl/JJyBlQ} for motivation}.
\1 Since the behavior of the network is dependent on other flows and packets, cannot easily decouple parts of the network.
\end{outline}

\subsection{What we want to solve}
\begin{outline}
\1 Want to provide network administrators with a tool for checking invariants before deploying network.
    \2 Also allow checking what happens in specific failure conditions (\eg if the network administrator knows that a particular middlebox is prone to failure).
    \2 \fixme{Check with Mooly and Z3 that this actually behaves reasonably} Also check what happens with partial failures or k-total failures automatically; can check if some failure causes problems.
\1 Assuming that we cannot  model the complete behavior of each middlebox, so we are not trying to model the complex classification algorithm, and instead rely on a classification oracle.
    \2 Verification is for invariants expressed in terms of the result of this oracle.
\1 For these networks we are primarily trying to check isolation (\ie can packets/data be accessed from certain places).
    \2 Security is one of the primary reasons for adding middleboxes, hence makes sense.
\end{outline}

\subsection{Some issues with our solution}
\begin{outline}
\1 We require models of middleboxes to be provided as input. Correctness is modulo models being correct, and the granularity of verification is affected by models.
\1 To achieve scalability when building such a tool we give up some soundness, \ie our tool will sometimes indicate invariant violation when none exist.
    \2 In particular we don't understand the semantics of an Oracle, so cannot easily reason about cases where the function keeps traffic safe. 
    \2 Also do not understand semantics of changed packet fields: we treat the packet fields symbolically and the processing is symbolic, will sometimes trigger a false alarm when accessing a changed field.
\1 For scalability also need to assume something about the network structure
    \2 A given packet can only go to a certain set of middleboxes. This set is smaller than the entire network.
        \3 When testing in the presence of failures, this must hold even 
    \2 This property is useful in general \fixme{\ldots}
\1 We do not address performance at all.
    \2 \fixme{My private conversations with both Google and Microsoft revealed it was very hard to get them to even specify the performance problem in a way that we could attempt to verify this}.
\end{outline}

==> outline.tex <==
\section{Outline}
\begin{outline}
\1 Related Work
\1 Conclusion
\end{outline}

==> rono.tex <==
\section{Scaling Verification}
\label{sec:scalability}
While the procedure outlined in \secref{sec:system} can produce formulas for verifying invariants in a weak logic,
scalability remains an important challenge. We need to ensure that verification is fast enough to be useful to network operators,
even when dealing with very large networks. Furthermore, since checking satisfiability is undecidable in general, SMT solvers eventually
timeout and might not be able to prove (or disprove) satisfiability even when a formula belongs to a decidable logic. Scaling verification
is therefore crucial for successfully verifying invariants on large networks.

Compositional verification provides an avenue for scalability by allowing us to prove properties on small subsets of a network and combine these
proofs to show that an invariant holds for the whole network. More formally, compositional verification allows us to compose the proof $N_1\Rightarrow I_1$ (\ie
invariant $I_1$ holds for network $N_1$) and $N_2\Rightarrow I_2$ to derive that both $I_1$ and $I_2$ hold for $N_1\cup N_2$\footnote{We define the union of two 
networks to be the network formed by taking the union of nodes and links from both networks.}, \ie  $N_1\cup N_2\Rightarrow I_1\cap I_2$. In general, compositional reasoning cannot be used to verify reachability invariants for networks.
Here we present \emph{cRONO}, a set of sufficient conditions for networks, that enables compositional verification of reachability invariants.

Before deriving conditions for a network to be cRONO, we define abstract semantics for middleboxes.\footnote{As opposed to the logical models from \secref{sec:system}, these semantic models allows us to reason about statements that hold
for all middleboxes, rather than for an individual type.} Our semantic model generalizes transfer functions (\secref{sec:system:transfer}) by adding a notion of history.
We define a middlebox's semantic function over a potentially infinite set of located packets $P$ and the set of (potentially unbounded) sequences of packets 
$P^*$.  A middlebox $m$ is the function $m: P\times P^* \rightarrow 2^P$, \ie $m$ takes as input a packet ($p\in P$) and a history of packets previously seen by
this middlebox $h\in P^*$ and outputs a (possibly empty) set of packet $m(p, h)$.  %\fixme{I feel we haven't emphasized this history enough early in the paper}

A \emph{cRONO} network is built up of middleboxes that are either \emph{RONO} or \emph{eRONO}. We start by precisely defining the properties of RONO and eRONO
middleboxes. We say a middlebox is RONO if it partitions its state between flows, such that its behavior for a packet $p$ depends only on the history of 
packets belonging to the same flow as $p$, \ie middlebox $m$ is RONO if and only if 
$\forall p\in P, h\in P^*:\, m(p, h) = m(p, h|_{flow(p)})$, where $h|_{flow(p)}$ is the subsequence of the history $h$ containing only those 
packets which belong to the same flow as $p$. When a network $N$ contains exactly one middlebox $m$ (and many switches and end hosts), then if $m$ is RONO, 
reachability invariants for $N$ can be verified compositionally.

\begin{figure}[tb]
\centering
\subfigure[]{
  \centering
  \includegraphics[width=0.3\textwidth]{figs/lan_1fw}
% \caption{Topology for enterprise network. $f$ is a hole-punching firewall, $d_k$, $h_k$ and $b_k$ are three different classes of hosts.}
   \label{fig:enterprise}
}
\hfill
\subfigure[]{
  \centering
  \includegraphics[width=0.35\textwidth]{plots/singlefw_combined}
%   \caption{Time taken to check that all nodes in a network satisfy appropriate invariants. y-axis is in log scale}
    \label{fig:singlefw_pipe}
}
\caption{\subref{fig:enterprise} Topology for an enterprise network: $f$ is a whole punching firewall, $e_k$, $h_k$ and $q_k$ are different classes of hosts; \subref{fig:singlefw_pipe}  average verification time per invariant.}
\vspace{-0.1in}
\label{fig:singlefw_all}
\end{figure}

While middleboxes such as learning firewalls, application firewalls etc. can be RONO, content-caches are not RONO; whether a content cache returns a cached result
or not depends on whether any end host has previously requested the same content. However, what is required for compositional verification of reachability
invariants is that a middlebox exhibit the same set of behaviors in a subset of the network as it does in the whole network. For example, in the presence
of a content cache $C$, end host $A$'s request for content $c$ might be served from the cache due to a previous request by $B$. If we consider the subnetwork 
without $B$, $A$ could still replicate this behavior by making two requests for content $c$; the second of which will be served from the cache.
Formally, a middlebox is \emph{extended RONO} (\emph{eRONO}) if and only if: $$\forall p, h:\, \exists h'\supseteq h|_{flow(p)}\, m(p, h) = m(p, h'|_{flow(p)})$$  \ie for any behavior exhibited by the middlebox for a packet $p$ we can find an alternate history $h'\supseteq h|_{flow(p)}$ which extends $h_{flow(p)}$ and
for which the same behavior is exhibited when only packets belonging to the same flow as $p$ are considered.

As previously shown (\secref{sec:modeling:rono}), the combination of several eRONO middleboxes might not be eRONO, \ie we cannot necessarily apply compositional
verification to a network of several eRONO middleboxes. We define \emph{Compositional RONO} (cRONO) middleboxes to be middleboxes whose combination is guaranteed
to be amenable to compositional verification. The following is a list of sufficient conditions for a middlebox to be cRONO:
\begin{asparaenum}
\item The middlebox is \emph{eRONO}.
\item The forwarding behavior of the middlebox is deterministic with respect to flows, \ie for cRONO middlebox $m$:
     $$\forall p, h, h':\, h|_{flow(p)} = h'|_{flow(p)} \implies m(p, h) = m(p, h')$$
\item The middlebox either drops all packets belonging to the same flow, or none of them. Further, all packets belonging to the same flow must be forwarded 
to the same set of locations, \ie if $loc(p)$ denotes the set of locations output by the middlebox then:
\begin{align*}
\forall p, p', h:&\ flow(p) = flow(p') \implies\\
   &loc(m(p, h)) = loc(m(p', h\cup{p}))
\end{align*}
\item The middlebox preserves flows, \ie it never merges two flows:
\begin{align*}
\forall p, p', h, h':&\ flow(m(p, h)) = flow(m(p', h'))\\
   &\iff flow(p) = flow(p')
\end{align*}
\end{asparaenum}
It is simple to see that with these conditions any combination of \emph{cRONO} middleboxes is itself \emph{cRONO}, 
and we refer to such a combination as a \emph{cRONO} network.

A network being \emph{cRONO} is a sufficient condition for applying compositional reasoning, however it is not a necessary condition.
For example, content caches are \emph{not} cRONO. However, in the cache and firewall example from \secref{sec:modeling:rono} (Figure~\ref{fig:ronoeg}),
we can apply compositional reasoning as long as the cache can enforce ACLs\footnote{This is true for common
caches such as Squid, Apache Web Proxy, nginx, etc.}, and the set of ACLs enforced by the cache is a superset of those enforced by
the firewall.

In \secref{sec:eval} we show that compositional verification is essential for applying \name to large networks; we show that verification time
can improve by up to $125\times$ when invariants are verified compositionally.

% \begin{table}[tb]
% \centering
% \begin{tabular}{|l|r|r|}
% \hline
% Hosts & Firewall & Content Cache\\
% \hline
% $500$ & $43.87$s & $282.94$s \\
% $1000$ & $384.15$s & $4264.16$s\\
% $1500$ & $1736.70$s & $19819.72$s\\
% \hline
% \end{tabular}
% \caption{Time to verify invariants in larger
% networks.}
% \vspace{-0.1in}
% \label{tab:largeverification}
% \end{table}


==> tractability.tex <==
% \notepanda{See if we can do better here.}
\eat{
Next we try and answer two questions about our formulation: are our formulas decidable (\secref{sec:tractability:decidability}) \ie can Z3 solver find a satisfiable assignment (or prove that the formulas are unsatisfiable) in a finite number of steps, and secondly conditions under which combination of middleboxes will result in RONO pipelines (\secref{sec:tractability:rono}).
}

% in \secref{sec:tractability:decidability} we show that checking isolation invariants is decidable given middleboxes and topologies are restricted
% in the manner described in \secref{sec:system}. 

% Next we analyze, theoretically, some of the properties of our system and formulation. We begin by showing (\secref{sec:tractability:decidability}) that verifying 
% isolation invariants is decidable in our formulation. This shows that even for middleboxes which we have not evaluated (or
% for new middleboxes which do not yet exist) we can verify isolation invariants as long as the conditions in \secref{sec:system} 
% are met. Next (\secref{sec:tractability:rono}, we analyze requirements for combining flow-parallel middleboxes into RONO pipelines. Finally in \secref{sec:tractability:scalability} we provide some insight into scalability requirements for our verification problem.

\section{Decidability}
\label{sec:tractability}
As noted in \secref{sec:system}, first-order logic is undecidable. Further, verifying a network with mutable datapaths is undecidable in general, such networks are
Turing complete. However,
we believe that we can express networks obeying the following restrictions in a decidable fragment of first-order logic:
\begin{asparaenum}
\item All middleboxes used in the network are passive, \ie they send packets only in response to packets received by them. In particular this means
      that every packet sent by a middlebox is causally related to some packet previously sent by an end-host. 
\item A middlebox sends a finite number of packets in response to any packets it receives. 
\item All packet processing pipelines are loop free, \ie any packets that enter the network are delivered or dropped in a finite number of steps.
\end{asparaenum}

We now show that we can express middleboxes and networks meeting this criterion in a logic built by extending ``effectively propositional logic'' (\emph{EPR}). 
EPR is a fundamental, decidable fragment of first-order logic~\cite{JAR:PiskacMB10}, where all axioms are of the form $\exists^*\forall^*$, and the
invariant is of the form $\forall^*\exists^*$. Neither axioms nor invariants in this logic can contain function symbols. EPR-F extends EPR to allow some unary functions. To guarantee decidability, EPR-F requires that there exist a finite set of compositions of unary functions $U$, such that any composition of unary functions can be reduced to a composition in $U$. For example, when a single unary function $f$ is used, we require that there exist $k$ such that 
$f^k(x) = f^{k-1}(x)$ for all $k$. Function symbols that go from one type to another are allowed, as long as their inverse is not used~\cite{Korovin}
 (\eg we can use $\src$ in our formulas since it has no inverse). Prior work~\cite{Itzhaky:2014:MRH:2535838.2535854} has discussed mechanisms to reduce EPR-F formulas to EPR.

We can translate our models to EPR-F by:  \eat{and then use
the fact that our topology and middleboxes are loop-free to prove that the introduced functions enjoy the required closure property}
\begin{asparaenum}
\item Reformulate our assertions with ``event variables'' and functions that assign properties like time, source and destination to an event. We use predicate function to mark events
     as either being sends or receives.  
\item Replace $\forall\exists$ formulas with equivalent formulas that contain Skolem functions instead of symbols.
\end{asparaenum}

For example the statement 
$$\forall d,s,p\, : 
\rcv(d, s, p) \implies \past{\snd(s, d, p)}$$
is translated to the formula $$\forall e\, : rcv(e) \Rightarrow snd(cause(e)) \land \ldots \land t(cause(e)) < t(e)$$ 
We also add the axiom,  $\forall e: snd(e) \Rightarrow cause(e) = e$  which says that a $snd$ event has no cause, ensuring idempotency.

To show that our models are expressible in EPR-F, we need to show that all unary functions introduced during this conversion
meet the required closure properties. Intuitively, all function  introduced by us track the causality of network events. Our decidability
criterion imply that every network event has a finite causal chain. This combined with the axiom that $cause(e)$ is idempotent implies that
the functions meet the closure properties. However, for Z3 to guarantee termination, explicit axioms guaranteeing closure must be provided.
Generating these axioms from a network is left to future work. In our experience, Z3 terminates on networks meeting our criterion even in the
absence of closure axioms.


\eat{
\begin{figure}[tb]
\centering
\begin{flalign*}
    snd(e) \land s(e) = f &\implies t(cause(e)) < t(e)\\
                    &\land rcv(cause(e)) \\ 
                    &\land d(cause(e)) = f \\
                    & \land p(cause(e)) = p(e) \\
                    & \land acl(s(e1), d(e1)) \\
    rcv(e) \lor s(e) \neq f &\implies cause(e) = e 
\end{flalign*}
\caption{EPR-F formulas equivalent to \\
$send(f, n, p, t) \Rightarrow (\exists t', n'. recv(n', f, p, t') \land t' < t \land acl(s(p), d(p))$.\noteori{fix this to translate the temporal formula}}
\label{fig:aclfwevformula}
\vspace{-0.1in}
\end{figure}
%\fixme{0.75 pages?}

In general, first order logic is undecidable. However we show that when we restrict our models (\secref{sec:system:modeling}) and topology (\secref{sec:system:transfer}) as described
previously, we get formulas that lie in a decidable fragment of first-order logic.
This fragment is a simple extension of ``effectively propositional logic" (\emph{EPR}). EPR is one of the fundamental decidable fragments of first-order logic~\cite{JAR:PiskacMB10}.
An EPR formula is a set of function symbol free $\exists^*\forall^*$ premises (assertions) and a function symbol free $\forall^*\exists^*$ formula as a consequence (whose negation 
is added as an assertion before checking for satisfiability). Z3 and other SMT solvers use algorithms that are guaranteed to terminate for this fragment. 

In our case, some of the formulas obtained from modeling middleboxes (\eg Figure~\ref{fig:fwformula}) as well as one of the network axioms (assertion 3 in Figure~\ref{fig:general}) are $\forall^*\exists^*$ premises and hence not in EPR. Therefore our case requires a more expressive logic that we call EPR-F. This logic extends EPR to allow restricted
unary functions. To ensure that the formulas are decidable, EPR-F requires that unary functions have certain closure properties ensuring that a finite set of compositions of these functions always suffices to express any other composition (including compositions of the function with itself), \eg for a EPR-F signature with a single function $f$ there must exist $k$ such that $f^k(x) = f^{k-1}(x)$.
Note that ``non-cyclic" function symbols that go from one type to another, while assuming that no function can go back, may be employed freely~\cite{Korovin}.
A fragment similar to EPR-F (but slightly more restrictive) was employed in \cite{Itzhaky:2014:MRH:2535838.2535854}, which also shows how such formulas can be reduced to pure EPR. 

One can translate our models (\eg Figure~\ref{fig:fwformula}) to EPR-F using the following steps and then use
the fact that our topology and middleboxes are loop-free to prove that the introduced functions enjoy the required closure property:
\begin{asparaenum}
\item Reformulate our assertions with ``event variables'' and functions that assign properties like time, source and destination to an event. We use predicate function to mark events
     as either being sends or receives.  \eat{For example we translate the formula $\forall n, n', p, t\, . recv(n, n', p, t)\implies \exists t'\,. send(n, n', p, t') \land t' < t$ to the equivalent formula
     $\forall e\, . rcv(e) \implies \exists 'e\, . snd(e) \land s(e) = s(e') \land d(e) = d(e') \land t(e') < t(e)$.}
\item Replace $\forall\exists$ formulas with equivalent formulas that contain Skolem functions instead of symbols. \eat{For instance the above formula is converted to 
$\forall e\, . rcv(e) \implies snd(cause(e)) \land \ldots \land t(cause(e) < t(e)$ where $cause$ is an uninterpreted unary function. Further, we add a second constraint saying that $\forall e\, . snc(e) \implies cause(e) = e$ (or 
equivalently that $cause(e)$ is idempotent for events that are not $rcv$ events. }%I ate this bit, mostly to see if it helps with space. Not yet sure what will happen.}
\end{asparaenum}
%For example the formula $\forall n, n', p, t\, . recv(n, n', p, t)\implies \exists t'\,. send(n, n', p, t') \land t' < t$ is translated to the equivalent formula $\forall e\, . rcv(e) \implies snd(cause(e)) \land \ldots \land t(cause(e)) < t(e)$ and we add a second assertion $\forall e\, . snd(e) \implies cause(e) = e$ to ensure that $cause(e)$ is idempotent for send events.
For example the statement 
$$\forall d,s,p\, . 
\rcv(d, s, p) \implies \past{\snd(s, d, p)}$$
is translated to the equivalent formula $$\forall e\, . rcv(e) \implies snd(cause(e)) \land \ldots \land t(cause(e)) < t(e)$$, and we add a second assertion $\forall e\, . snd(e) \implies cause(e) = e$ to ensure that $cause(e)$ is identity for send events (and hence, idempotent for all events).
Figure~\ref{fig:aclfwevformula} shows another example of this reformulation for a simple ACL firewall (with no learning action).

Finally, we need to show that any newly introduced unary functions have the desired closure properties. Note first that each cause functions is idempotent: they are the identity function for either send
or receive events and when not the identity function $cause$ links a send to a receive.
Furthermore, when applied to an event $e$ the value of this function (when not idempotent) is always another event such that $d(e) = s(e)$. Since the axioms ensure that forwarding is loop free, this must terminate
in a finite number of steps (when we would have reached the edge of the network) and therefore the newly introduced functions meets the requirement for being in EPR-F.
 }
%  functions assigns a previous event whose destination is the source of the current event. In other words,
% the introduced functions respect the network's topology. Assuming that the topology is loop free (see Section~\ref{sec:system:transfer}), one obtains a bound on the length of function 
% compositions that can lead to new events.

% \noteori{does this hold for the cache functions as well? maybe we should find a safer phrasing here.}

% \noteori{Is this clear at all???}


% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.94\columnwidth]{figs/fw_tractable}
% \caption{An example showing a finite number of instances for a network with a single firewall.}
% \label{fig:fw-tractable}
% \end{figure}
% \eat{
% \begin{outline}
% \1 Many kinds of middleboxes, tested here on a limited set.
%     \2 Works for our examples but what about other middleboxes and other topologies.
% \1 Want to show that given a loop free network topology, middleboxes using our limited grammar, a sufficiently good SMT solver and sufficient time we can
%   always compute whether isolation invariants hold.
%      \2 In general, formulas can be undecidable, so the proble is to show that our grammar can be converted to a set of formulas that can be decided.
%      \1 Describe Ori's form with events and functions.
% \1 In previous function, formulas are decidable if all finite composition of cause functions are equivalent to the identity function.
%     \2 For a single middlebox (for instance a firewall shown in Figure~\ref{fig:fw-tractable}) the lack of loops, and limited grammar makes this true.
%     \2 When composing middleboxes in a loop-free network eventually composition of functions gets us back to an endhost (at which point cause is identity function).
% \1 Thus there is a decidable form.
% \end{outline}
% }}
%%% Here lie dragons


